Exploring the Reasoning Abilities of Multimodal Large Language Models (MLLMs): A Comprehensive Survey on Emerging Trends in Multimodal Reasoning

Strong Artificial Intelligence (Strong AI) or Artificial General Intelligence (AGI) with abstract reasoning ability is the goal of next-generation AI. Recent advancements in Large Language Models (LLMs), along with the emerging field of Multimodal Large Language Models (MLLMs), have demonstrated impressive capabilities across a wide range of multimodal tasks and applications. Particularly, various MLLMs, each with distinct model architectures, training data, and training stages, have been evaluated across a broad range of MLLM benchmarks. These studies have, to varying degrees, revealed different aspects of the current capabilities of MLLMs. However, the reasoning abilities of MLLMs have not been systematically investigated. In this survey, we comprehensively review the existing evaluation protocols of multimodal reasoning, categorize and illustrate the frontiers of MLLMs, introduce recent trends in applications of MLLMs on reasoning-intensive tasks, and finally discuss current practices and future directions. We believe our survey establishes a solid base and sheds light on this important topic, multimodal reasoning.

==> Table/InfiMM.tex <==
\begin{table*}[htbp]
    \centering
    \caption{Evaluation results for various MLLMs. Open-source models best performances are indicated with underlines.}
    \resizebox{\textwidth}{!}{
    \setlength{\tabcolsep}{6pt}
    \begin{tabular}{lll|ccc|cc|c}
    \toprule

     \rowcolor{gray!20}  &  & & \multicolumn{3}{c|}{Reasoning Category} &\multicolumn{2}{c|}{Reasoning Complexity}&  \\
     \rowcolor{gray!20}\multirow{-2}{*}{MLLMs}& \multirow{-2}{*}{LLM}& \multirow{-2}{*}{IFT} & Deductive & Abductive & Analogical & Moderate & High & \multirow{-2}{*}{Overall} \\
    \midrule 
         OpenFlamingo-v2~\cite{awadalla2023openflamingo} & MPT-7B~\cite{mpt-7b} & No & 8.88 & 5.3 & 1.11 & 9.47 & 4.72& 6.82 \\
         MiniGPT-v2~\cite{zhu2023minigpt} &LLaMA2-7B~\cite{touvron2023llama} &Yes & 11.02 & 13.28 & 5.69 & 14.45 & 7.27& 10.43 \\
         Fuyu-8B~\cite{fuyu-8b} &Persimmon-8B~\cite{persimmon-8b} &No & 16.42 & 21.49 & 7.78 & 23.06 & 9.91& 15.7 \\
         BLIP-2~\cite{li2023blip2}  &OPT-2.7B~\cite{zhang2022opt} & No & 22.76 & 18.96 & 7.5 & 24.05 & 14.18& 19.31 \\
         InternLM-XComposer-VL~\cite{zhang2023internlmxcomposer} & InternLM-7B ~\cite{2023internlm} & Yes & 26.77 & 35.97 & 18.61 & 39.13 & 17.18& 26.84 \\
         InstructBLIP~\cite{chung2022scaling} &FLAN-T5-XXL~\cite{chung2022scaling}  & Yes& 27.56 & 37.76 & 20.56 & 40.64 & 18.09& 28.02 \\
         LLaMA-Adapter V2~\cite{gao2023llamaadapter} & LLaMA-7B~\cite{touvron2023llama} & No & 28.7 & 46.12 & 22.08 & 41.33 & 21.91& 30.46 \\
         Otter~\cite{li2023otter}  &LLaMA-7B  & Yes & 22.49 & 33.64 & 13.33 & 35.79 & 12.31 & 22.69 \\
         mPLUG-Owl2~\cite{ye2023mplugowl2} & LLaMA-7B & Yes  & 23.43 & 20.6 & 7.64 & 28.79 & 13.18 & 20.05 \\
         IDEFICS-9B-instruct~\cite{laurenccon2023obelisc} &LLaMA-7B & Yes & 22.99 & 34.63 & 20.56 & 34.45 & 16.73& 24.53 \\
         Emu~\cite{sun2023generative} & LLaMA-13B & Yes & 28.9 & 36.57 & 18.19 & 36.18 & 22.0 & 28.24 \\
         LLaVA-1.5~\cite{liu2023llava} & Vicuna-13B~\cite{vicuna2023} & Yes & 30.94 & \textbf{\underline{47.91}} & 24.31 & 47.4 & 21.0& 32.62 \\
         CogVLM-Chat~\cite{wang2023cogvlm} & Vicuna-7B & Yes & 36.75 & 47.88 & 28.75 & \textbf{\underline{55.67}} & 22.5& 37.16 \\
         Qwen-VL-Chat~\cite{bai2023qwenvl} &Qwen-14B \cite{Qwen-VL} & Yes & \textbf{\underline{37.55}} & 44.39 & \textbf{\underline{30.42}} & 46.61 & \textbf{\underline{30.09}} & \textbf{\underline{37.39}} \\
         \midrule
         GPT-4V~\cite{openai2023gpt4} &GPT-4 & Yes & \textbf{74.86} & \textbf{77.88} & \textbf{69.86} & \textbf{93.98} & \textbf{58.98} & \textbf{74.44} \\
    \midrule 
    \bottomrule
    \end{tabular}}
    \label{tab:main_result}
\end{table*}
